Gender-dependent Contribution, Code and Creativity in a Virtual Programming Course

Since computer science is still mainly male dominated, academia, industry and education jointly seek ways to motivate and inspire girls, for example by introducing them to programming at an early age. The recent COVID-19 pandemic has forced many such endeavours to move to an online setting. While the gender-dependent differences in programming courses have been studied previously, for example revealing that girls may feel safer in same-sex groups, much less is known about gender-specific differences in online programming courses. In order to investigate whether gender-specific differences can be observed in online courses, we conducted an online introductory programming course for Scratch, in which we observed the gender-specific characteristics of participants with respect to how they interact, their enjoyment, the code they produce, and the creativity exposed by their programs. Overall, we observed no significant differences between how girls participated in all-female vs. mixed groups, and girls generally engaged with the course more actively than boys. This suggests that online courses can be a useful means to avoid gender-dependent group dynamics. However, when encouraging creative freedom in programming, girls and boys seem to fall back to socially inherited stereotypical behavior also in an online setting, influencing the choice of programming concepts applied. This may inhibit learning and is a challenge that needs to be addressed independently of whether courses are held online.

==> detailsSessions.tex <==
\begin{table*}[tb]
\centering
\small
\caption{Details of the implementation of the concepts for each session.}
\label{tab:sessions}
\begin{tabular}{lllp{3cm}lp{3cm}p{1.5cm}}

\toprule
session & concept & topic & sprites & stages & block categories & project type \\ 
\midrule
1 & basics & magical forest & wizard, rabbit & forest & events, motion, looks, control, sound, text to speech & story \\
2 & loops & milk-dance & milk, radio & spotlight & events, control, sound, looks & animation \\
   &  & polar bear and penguin & polar bear, penguin & slopes & events, looks, motion, pen, control & story \\
3 & conditional  & talking dog & dog & white stage & event, sensing, looks, operators, control & story \\
   & statements & flying cat & cat, sun, cloud, line, balloon & blue sky & event, control, motion, sensing, looks & game \\
4 & conditional loops & catch game & cat, mouse, chick &  & motion, looks, events, control, sensing & game \\
5 & variables & happy hippo & hippo, spaceship, lightning & stars & event, looks, motion, operators, sensing, control, variables & game \\
   &  & tree watering & tree, cloud, rain drops (painted) & desert & event, looks, motion, operators, sensing, control, variables & game \\
6 & recap & my world & ball, beetle, dot, sign (painted), obstacles (painted), goal (painted) & grey stage & motion, looks, sound, events, control, sensing, operators, variables & animation/ game 
\\ \bottomrule

\end{tabular}
\end{table*}

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Correlation between contribution and outcome} %RQ1 und RQ3

One of the major challenges in a virtual setting is the lack of controllability as to whether students are actually following exactly what they are supposed to~\cite{hermans2017b}. Similar to the physical classroom, the assumption is that students who participate little and are distracted will also have poorer results than those who actively participate~\cite{gonzalez2012,zhan2015}.

In team and group tasks, it is often the case that girls, due to their low self-confidence, are more likely to designate boys as team leads and participate less~\cite{mcdowell2006, papavlasopoulou2020a}. Our results showed that girls do not let boys hold them back in a virtual setting and not only take the lead (\Cref{tab:studentCategory}), but also participate in general considerably more often than boys (\Cref{sec:rq1}).

Similarly, girls also have more correctly implemented programming concepts than boys (\Cref{sec:rq3}). 
The number of correctly implemented programming concepts goes down from session three for both genders and the questions increase for both genders from this session, especially for girls (\Cref{fig:qa}, \Cref{fig:taskcorrectsex}).


\subsection{Correlation between interest and outcome} % RQ2 und RQ3
It is well established that if you are interested in something and enjoy it, you will be more engaged and put more effort into it~\cite{mitchell1993, teague2002, ccakir2017}. Therefore, we consider the correlation of interest (\Cref{sec:rq2}) and the programs (\Cref{sec:rq3}).

Regarding the students' self-concept, it is interesting to note that the same number of both genders have engaged a little bit with \Scratch and girls have indicated less to engage often with it (REF POLLS), when the implementation of the additional tasks and additional projects shows us that girls have engaged more with \Scratch in their account across the board~\Cref{fig:addtaskcomparison}.

\subsection{Learning objectives}

Girls require different learning stimuli than boys because they have different expectations~\cite{rubio2015}. In particular, they value quick positive feedback~\cite{vrieler2020} that our course design attempted to optimize. The results show that the learning curve was chosen correctly and thus especially the girls remained interested. 

Across all groups, it is evident that there is a significant decrease in participation from the fourth session onwards. In particular, there are the least responses here (excluding lesson 6, which is not evaluated because there was little interaction here). 
This suggests that the introduction of conditional repetition is a difficult concept for students. Likewise, this may be related to the learning curve, which was very steep at the beginning. 
Furthermore, the motivation of the students might have decreased, since the conditional repetition is a combination of the previous concepts and does not provide a clearly recognizable added value than, for example, the variables in the fifth lesson with which new possibilities such as scoring were created. 

In general, there was little interaction between the students and in principle, communication was almost exclusively with the course leader. Even in the specially designed small groups in the breakout sessions, in which the students also showed their programs, there was hardly any interaction.
Individual observations in the groups were apparent, in which one student was helped with a problem by another student and thus the supervisor did not have to intervene.

\subsection{Changing Attitudes}
As a continuation of this course, special parent-child courses could follow. 
Many parents often have misconceptions about programming and computer science, so it could be helpful to convince them as well, as a student from the all-girls group said in the last session "There is a continuation? My father said I should do that, my mother said that will definitely not interest me" (12f).
This would also have the side effect of parent-child bonding, which can increase students' self-confidence.

The concept of small groups has also proven to be useful, so that everyone receives individual attention and the inhibition threshold when showing their own program is not too high. This presentation of one's own developed program can also serve as a motivator and support for self-efficacy. Working in small groups can be clarified with the concept of pair programming, which has already been shown in some small studies~\cite{lewis2015, zhong2016, papadakis2018a, ying2019} and be implemented more in primary education in particular.

After a certain age or level of experience, same-sex courses might not seem useful, as this will only increase the discrepancy and antipathy between girls and boys. Similarly, this could skew the challenges in practice when, in everyday work, most software teams are made up of men. One area of application, however, would be in introductory programming courses at university, for example, since girls without prior experience might also feel intimidated by knowledge already acquired by their male fellow students~\cite{ying2019}.

==> metricSex.tex <==
\begin{table}[tb]
\centering
\caption{Metrics for female and male students in total.}
\label{tab:metricstotal}
\begin{tabular}{lrr}

\toprule
Metric & Female & Male \\ 
\midrule
%contributions & 407 & 435 \\
%answers & 138 & 126 \\
%questions & 269 & 309 \\
correct tasks & 206 & 194 \\
incorrect tasks & 14 & 22 \\
missing tasks & 44 & 83 \\
additonal tasks & 76 & 57 \\
no additonal tasks & 122 & 171 \\
additonal sprites & 104 & 83 \\
no additonal sprites & 160 & 221 \\ 
\bottomrule
\end{tabular}
\end{table}

==> relatedwork.tex <==
\section{Related Work}
\label{sec:rw}




==> resultsProjects.tex <==
\begin{table}[tb]
    \centering
    \caption{Evaluation of the programs for each task regarding correctness, availability, homework and creativity. \small There are 71 participants in total (f: 33, m: 88), hence potentially 71 projects per task.}
    \label{tab:resultsProjects}
    \begin{tabular}{lrrrrrrrrr}
   
    \toprule
        metric & 1 & 2.1 & 2.2 & 3.1 & 3.2 & 4 & 5 & 6 \\ 
     \midrule
     
        task: correct F & 28 & 31 & 28 & 28 & 29 & 21 & 24 & 17 \\ 
        task: correct M & 32 & 27 & 24 & 23 & 26 & 24 & 21 & 17 \\ 
        task: missing total V & 19 & 15 & 24 & 27 & 22 & 37 & 32 & 46 \\ 
        task: missing F V & 7 & 4 & 7 & 7 & 5 & 12 & 10 & 20 \\ 
        task: missing M V & 12 & 11 & 17 & 20 & 17 & 25 & 22 & 26 \\ 
        task: missing total I & 10 & 7 & 14 & 19 & 13 & 21 & 17 & 24 \\ 
        task: missing F & 5 & 1 & 3 & 5 & 3 & 11 & 4 & 10 \\ 
        task: missing M & 5 & 6 & 11 & 14 & 10 & 10 & 13 & 14 \\ 
        add: done total & 41 & - & 5 & - & 10 & 28 & 23 & 26 \\ 
        add: done F & 23 & - & 3 & - & 6 & 17 & 15 & 12 \\ 
        add: done M & 16 & - & 2 & - & 4 & 12 & 11 & 16 \\ 
        sprites: total & 14 & 32 & 4 & 29 & 11 & 33 & 31 & 33 \\ 
        sprites: total F & 9 & 14 & 3 & 18 & 8 & 17 & 19 & 16 \\ 
        sprites: total M & 5 & 18 & 1 & 11 & 3 & 16 & 12 & 17 \\ 
        
        \bottomrule
        
\end{tabular}
\end{table}

==> studentCategory.tex <==
\begin{table}[tb]
\centering
\caption{Top five participations of each student and category.}
\label{tab:studentCategory}
\begin{tabular}{rrlrlrlrl}

\toprule
{} &  \# A  &   \allfemale (A) &  \# B  &   \allmale (B) &  \# C  &   \mixed (C) &  \# D  &   \mixed (D) \\
\midrule
1  &     44 &      12f - question 		&     39 &     22m - question 		&     50 &       49f - question 		&     27 &        85m  - question \\
2  &     21 &      12f - answer 		&     20 &       45m - question 		&     16 &		95m - question 	&     23 &            86f - question \\
3  &     15 &         07f - answer 	&     16 &         21m - question 		&     11 &      47f - answer 		&     22 &                86f - answer \\
4  &     14 &      05f - question &     16 &        38m - answer 	&      9 &      54m - question 	&     19 &     76m - question \\
5  &     14 &      07f - reaction 		&     14 &        24m - question 	&      8 &         56m - answer 	&     11 &          93f - question \\
%6  &     12 &     01f - reaction 	&     13 &           23m - answer 		&      8 &        56m - question 	&     11 &        85m - question \\
%7  &     11 &     16f - question &     12 &          22m - chitchat 	&     7 &      58m - answer 	 &     10 &      76m - answer \\
%8  &     10 &        01f - question 	&     11 &     34m - answer 	&     	 7 &       49f  - answer		&     10 &            61m - question \\
%9  &      9 &       05f - reaction 	&      9 &               27m - question 		&      	7 &      58m - question 	&      9 &        84f - question \\
%10  &      8 &       05f - answer 	&      9 &          22m - answer 		&     6 &	  42f - answer 		&      7 &               86f - chitchat \\

\bottomrule

\end{tabular}
\end{table}
